Query Embedding on Hyper-relational Knowledge Graphs

Multi-hop logical reasoning is an established problem in the field of representation learning on knowledge graphs (KGs). It subsumes both one-hop link prediction as well as other more complex types of logical queries. Existing algorithms operate only on classical, triple-based graphs, whereas modern KGs often employ a hyper-relational modeling paradigm. In this paradigm, typed edges may have several key-value pairs known as qualifiers that provide fine-grained context for facts. In queries, this context modifies the meaning of relations, and usually reduces the answer set. Hyper-relational queries are often observed in real-world KG applications, and existing approaches for approximate query answering cannot make use of qualifier pairs. In this work, we bridge this gap and extend the multi-hop reasoning problem to hyper-relational KGs allowing to tackle this new type of complex queries. Building upon recent advancements in Graph Neural Networks and query embedding techniques, we study how to embed and answer hyper-relational conjunctive queries. Besides that, we propose a method to answer such queries and demonstrate in our experiments that qualifiers improve query answering on a diverse set of query patterns.

==> generated/baseline_AMRI.tex <==
% >>> AMRI <<<
% \begin{tabular}{llllllll}
% \toprule
% {} & \multicolumn{1}{c}{\texttt{1p}} & \multicolumn{1}{c}{\texttt{2p}} & \multicolumn{1}{c}{\texttt{3p}} & \multicolumn{1}{c}{\texttt{2i}} & \multicolumn{1}{c}{\texttt{3i}} & \multicolumn{1}{c}{\texttt{2i-1p}} & \multicolumn{1}{c}{\texttt{1p-2i}} \\
% \midrule
StarQE      &                         $78.44$ &                         $68.11$ &                         $74.62$ &                         $93.63$ &                         $98.65$ &                            $73.14$ &                            $88.76$ \\
Triple-Only &                         $88.14$ &                         $81.25$ &                         $95.92$ &                         $99.18$ &                         $99.95$ &                            $83.44$ &                            $98.91$ \\
Reification &                $\mathbf{88.81}$ &                         $86.63$ &                $\mathbf{96.20}$ &                $\mathbf{99.24}$ &                $\mathbf{99.96}$ &                            $85.46$ &                   $\mathbf{99.10}$ \\
Zero Layers &                         $88.03$ &                $\mathbf{90.56}$ &                         $95.79$ &                         $96.34$ &                         $98.37$ &                   $\mathbf{86.18}$ &                            $98.55$ \\
% \bottomrule
% \end{tabular}
% 


==> generated/baseline_H_at_1.tex <==
% >>> H@1 <<<
% \begin{tabular}{llllllll}
% \toprule
% {} & \multicolumn{1}{c}{\texttt{1p}} & \multicolumn{1}{c}{\texttt{2p}} & \multicolumn{1}{c}{\texttt{3p}} & \multicolumn{1}{c}{\texttt{2i}} & \multicolumn{1}{c}{\texttt{3i}} & \multicolumn{1}{c}{\texttt{2i-1p}} & \multicolumn{1}{c}{\texttt{1p-2i}} \\
% \midrule
StarQE      &                         $20.91$ &                $\mathbf{39.98}$ &                $\mathbf{45.85}$ &                $\mathbf{55.11}$ &                         $78.58$ &                   $\mathbf{51.77}$ &                   $\mathbf{65.77}$ \\
Base Triple &                         $11.62$ &                          $2.97$ &                          $7.57$ &                         $36.87$ &                         $64.72$ &                             $3.33$ &                            $13.00$ \\
Reification &                $\mathbf{24.26}$ &                         $38.82$ &                         $42.80$ &                         $49.67$ &                $\mathbf{78.93}$ &                            $42.39$ &                            $55.05$ \\
Zero Layers &                         $18.30$ &                         $12.92$ &                         $11.53$ &                         $40.35$ &                         $74.27$ &                            $18.17$ &                            $19.51$ \\
% \bottomrule
% \end{tabular}
% 


==> generated/baseline_H_at_3.tex <==
% >>> H@3 <<<
% \begin{tabular}{llllllll}
% \toprule
% {} & \multicolumn{1}{c}{\texttt{1p}} & \multicolumn{1}{c}{\texttt{2p}} & \multicolumn{1}{c}{\texttt{3p}} & \multicolumn{1}{c}{\texttt{2i}} & \multicolumn{1}{c}{\texttt{3i}} & \multicolumn{1}{c}{\texttt{2i-1p}} & \multicolumn{1}{c}{\texttt{1p-2i}} \\
% \midrule
StarQE      &                         $35.58$ &                $\mathbf{46.41}$ &                $\mathbf{57.34}$ &                         $67.98$ &                         $87.56$ &                   $\mathbf{56.89}$ &                   $\mathbf{75.35}$ \\
Base Triple &                         $25.54$ &                          $6.38$ &                         $15.44$ &                         $53.45$ &                         $81.55$ &                             $7.40$ &                            $23.56$ \\
Reification &                $\mathbf{40.12}$ &                         $45.58$ &                         $55.45$ &                $\mathbf{68.31}$ &                $\mathbf{89.84}$ &                            $51.33$ &                            $70.26$ \\
Zero Layers &                         $31.98$ &                         $21.34$ &                         $25.24$ &                         $55.83$ &                         $85.43$ &                            $25.75$ &                            $35.67$ \\
% \bottomrule
% \end{tabular}
% 


==> generated/generalization_AMRI.tex <==
% >>> AMRI <<<
% \begin{tabular}{llllllll}
% \toprule
% {} &     \multicolumn{1}{c}{\texttt{1p}} &     \multicolumn{1}{c}{\texttt{2p}} &     \multicolumn{1}{c}{\texttt{3p}} & \multicolumn{1}{c}{\texttt{2i}} & \multicolumn{1}{c}{\texttt{3i}} & \multicolumn{1}{c}{\texttt{2i-1p}} & \multicolumn{1}{c}{\texttt{1p-2i}} \\
% \midrule
StarE-like       &           \cellcolor{yellow}$78.44$ &           \cellcolor{yellow}$68.11$ &           \cellcolor{yellow}$74.62$ &       \cellcolor{yellow}$93.63$ &       \cellcolor{yellow}$98.65$ &          \cellcolor{yellow}$73.14$ &          \cellcolor{yellow}$88.76$ \\
Q2B-like         &           \cellcolor{yellow}$88.69$ &  \cellcolor{yellow}$\mathbf{87.17}$ &  \cellcolor{yellow}$\mathbf{95.60}$ &       \cellcolor{yellow}$99.01$ &       \cellcolor{yellow}$99.93$ &                            $83.24$ &                            $98.49$ \\
emQL-like        &           \cellcolor{yellow}$73.20$ &                             $51.74$ &                             $74.93$ &       \cellcolor{yellow}$90.68$ &                         $97.79$ &                            $37.80$ &                            $82.59$ \\
MPQE-like        &           \cellcolor{yellow}$93.77$ &                             $83.25$ &                             $92.00$ &                         $99.49$ &                         $99.96$ &                            $85.61$ &                            $99.04$ \\
MPQE-like + Reif &  \cellcolor{yellow}$\mathbf{95.68}$ &                             $82.93$ &                             $92.08$ &                $\mathbf{99.57}$ &                $\mathbf{99.97}$ &                   $\mathbf{86.54}$ &                   $\mathbf{99.25}$ \\
% \bottomrule
% \end{tabular}
% 


==> generated/generalization_H_at_1.tex <==
% >>> H@1 <<<
% \begin{tabular}{llllllll}
% \toprule
% {} &     \multicolumn{1}{c}{\texttt{1p}} &     \multicolumn{1}{c}{\texttt{2p}} &     \multicolumn{1}{c}{\texttt{3p}} &     \multicolumn{1}{c}{\texttt{2i}} & \multicolumn{1}{c}{\texttt{3i}} &  \multicolumn{1}{c}{\texttt{2i-1p}} &  \multicolumn{1}{c}{\texttt{1p-2i}} \\
% \midrule
StarE-like       &           \cellcolor{yellow}$20.91$ &  \cellcolor{yellow}$\mathbf{39.98}$ &  \cellcolor{yellow}$\mathbf{45.85}$ &  \cellcolor{yellow}$\mathbf{55.11}$ &       \cellcolor{yellow}$78.58$ &  \cellcolor{yellow}$\mathbf{51.77}$ &  \cellcolor{yellow}$\mathbf{65.77}$ \\
Q2B-like         &           \cellcolor{yellow}$21.63$ &           \cellcolor{yellow}$37.15$ &           \cellcolor{yellow}$43.82$ &           \cellcolor{yellow}$52.49$ &       \cellcolor{yellow}$77.36$ &                             $37.59$ &                             $59.74$ \\
emQL-like        &           \cellcolor{yellow}$23.06$ &                              $6.78$ &                             $19.86$ &           \cellcolor{yellow}$53.36$ &                $\mathbf{81.73}$ &                              $2.17$ &                             $48.54$ \\
MPQE-like        &           \cellcolor{yellow}$16.53$ &                              $3.81$ &                             $12.70$ &                             $41.01$ &                         $60.67$ &                              $6.84$ &                             $28.76$ \\
MPQE-like + Reif &  \cellcolor{yellow}$\mathbf{25.52}$ &                              $3.24$ &                             $10.52$ &                             $41.36$ &                         $63.93$ &                              $5.59$ &                             $18.75$ \\
% \bottomrule
% \end{tabular}
% 


==> generated/generalization_H_at_3.tex <==
% >>> H@3 <<<
% \begin{tabular}{llllllll}
% \toprule
% {} &     \multicolumn{1}{c}{\texttt{1p}} &     \multicolumn{1}{c}{\texttt{2p}} &     \multicolumn{1}{c}{\texttt{3p}} & \multicolumn{1}{c}{\texttt{2i}} & \multicolumn{1}{c}{\texttt{3i}} &  \multicolumn{1}{c}{\texttt{2i-1p}} &  \multicolumn{1}{c}{\texttt{1p-2i}} \\
% \midrule
StarE-like       &           \cellcolor{yellow}$35.58$ &  \cellcolor{yellow}$\mathbf{46.41}$ &  \cellcolor{yellow}$\mathbf{57.34}$ &       \cellcolor{yellow}$67.98$ &       \cellcolor{yellow}$87.56$ &  \cellcolor{yellow}$\mathbf{56.89}$ &  \cellcolor{yellow}$\mathbf{75.35}$ \\
Q2B-like         &           \cellcolor{yellow}$38.79$ &           \cellcolor{yellow}$43.75$ &           \cellcolor{yellow}$55.41$ &       \cellcolor{yellow}$67.02$ &       \cellcolor{yellow}$87.97$ &                             $46.99$ &                             $71.20$ \\
emQL-like        &           \cellcolor{yellow}$36.14$ &                             $10.73$ &                             $30.47$ &       \cellcolor{yellow}$66.56$ &                         $89.91$ &                              $3.80$ &                             $55.96$ \\
MPQE-like        &           \cellcolor{yellow}$30.82$ &                              $7.15$ &                             $21.48$ &                         $66.87$ &                         $86.17$ &                             $10.08$ &                             $44.88$ \\
MPQE-like + Reif &  \cellcolor{yellow}$\mathbf{41.26}$ &                              $6.34$ &                             $18.25$ &                $\mathbf{68.14}$ &                $\mathbf{90.07}$ &                              $8.56$ &                             $32.31$ \\
% \bottomrule
% \end{tabular}
% 


==> generated/relation-specific/all.tex <==
\begin{tabular*}{\linewidth}{l*{4}{rl@{\extracolsep{\fill}}}}
% \begin{tabular}{llr|lr|lr}
\toprule

{} & \multicolumn{2}{c}{AMRI} & \multicolumn{2}{c}{H@10} & \multicolumn{2}{c}{MRR} \\
pattern & \multicolumn{1}{c}{relation} & \multicolumn{1}{c}{improvement} &  \multicolumn{1}{c}{relation} & \multicolumn{1}{c}{improvement} &  \multicolumn{1}{c}{relation} & \multicolumn{1}{c}{improvement} & \\

\midrule

\parbox[t]{2mm}{\multirow{10}{*}{\rotatebox[origin=c]{90}{1hop}}} &    \href{https://www.wikidata.org/wiki/Property:P518}{P518} &   ${\color{red}-\phantom{0}5.24} \pm \phantom{0}2.09$ &  \href{https://www.wikidata.org/wiki/Property:P1264}{P1264} &  ${\color{blue}+\phantom{0}3.64} \pm \phantom{0}1.50$ &    \href{https://www.wikidata.org/wiki/Property:P518}{P518} &  ${\color{blue}+\phantom{0}2.88} \pm \phantom{0}0.86$ \\

&    \href{https://www.wikidata.org/wiki/Property:P453}{P453} &   ${\color{red}-\phantom{0}2.75} \pm \phantom{0}0.78$ &    \href{https://www.wikidata.org/wiki/Property:P453}{P453} &  ${\color{blue}+\phantom{0}6.00} \pm \phantom{0}2.70$ &    \href{https://www.wikidata.org/wiki/Property:P453}{P453} &  ${\color{blue}+\phantom{0}3.78} \pm \phantom{0}0.98$ \\

&  \href{https://www.wikidata.org/wiki/Property:P1264}{P1264} &   ${\color{red}-\phantom{0}0.02} \pm \phantom{0}0.42$ &    \href{https://www.wikidata.org/wiki/Property:P518}{P518} &  ${\color{blue}+\phantom{0}6.84} \pm \phantom{0}4.47$ &      \href{https://www.wikidata.org/wiki/Property:P17}{P17} &  ${\color{blue}+\phantom{0}4.12} \pm \phantom{0}1.23$ \\

&  \href{https://www.wikidata.org/wiki/Property:P1686}{P1686} &  ${\color{blue}+\phantom{0}0.30} \pm \phantom{0}1.45$ &      \href{https://www.wikidata.org/wiki/Property:P17}{P17} &  ${\color{blue}+\phantom{0}6.89} \pm \phantom{0}2.82$ &  \href{https://www.wikidata.org/wiki/Property:P3831}{P3831} &  ${\color{blue}+\phantom{0}4.56} \pm \phantom{0}0.97$ \\

&  \href{https://www.wikidata.org/wiki/Property:P2453}{P2453} &  ${\color{blue}+\phantom{0}0.62} \pm \phantom{0}0.59$ &    \href{https://www.wikidata.org/wiki/Property:P805}{P805} &  ${\color{blue}+\phantom{0}8.25} \pm \phantom{0}1.44$ &    \href{https://www.wikidata.org/wiki/Property:P805}{P805} &  ${\color{blue}+\phantom{0}4.67} \pm \phantom{0}0.50$ \\

&  \href{https://www.wikidata.org/wiki/Property:P2453}{P2453} &  ${\color{blue}+\phantom{0}0.62} \pm \phantom{0}0.59$ &    \href{https://www.wikidata.org/wiki/Property:P805}{P805} &  ${\color{blue}+\phantom{0}8.25} \pm \phantom{0}1.44$ &    \href{https://www.wikidata.org/wiki/Property:P805}{P805} &  ${\color{blue}+\phantom{0}4.67} \pm \phantom{0}0.50$ \\

&  \href{https://www.wikidata.org/wiki/Property:P3831}{P3831} &  ${\color{blue}+\phantom{0}1.89} \pm \phantom{0}1.01$ &  \href{https://www.wikidata.org/wiki/Property:P3831}{P3831} &  ${\color{blue}+\phantom{0}9.86} \pm \phantom{0}1.21$ &  \href{https://www.wikidata.org/wiki/Property:P1686}{P1686} &            ${\color{blue}+10.36} \pm \phantom{0}0.58$ \\

&    \href{https://www.wikidata.org/wiki/Property:P805}{P805} &  ${\color{blue}+\phantom{0}2.42} \pm \phantom{0}2.58$ &  \href{https://www.wikidata.org/wiki/Property:P1686}{P1686} &            ${\color{blue}+13.70} \pm \phantom{0}1.19$ &  \href{https://www.wikidata.org/wiki/Property:P1264}{P1264} &            ${\color{blue}+11.17} \pm \phantom{0}2.30$ \\

&      \href{https://www.wikidata.org/wiki/Property:P17}{P17} &  ${\color{blue}+\phantom{0}2.53} \pm \phantom{0}3.02$ &  \href{https://www.wikidata.org/wiki/Property:P1346}{P1346} &            ${\color{blue}+24.04} \pm \phantom{0}3.87$ &  \href{https://www.wikidata.org/wiki/Property:P1346}{P1346} &            ${\color{blue}+27.78} \pm \phantom{0}4.01$ \\

&  \href{https://www.wikidata.org/wiki/Property:P1346}{P1346} &  ${\color{blue}+\phantom{0}4.08} \pm \phantom{0}3.30$ &  \href{https://www.wikidata.org/wiki/Property:P2453}{P2453} &            ${\color{blue}+33.03} \pm \phantom{0}4.26$ &  \href{https://www.wikidata.org/wiki/Property:P2453}{P2453} &            ${\color{blue}+45.82} \pm \phantom{0}3.48$ \\

\midrule
\parbox[t]{2mm}{\multirow{10}{*}{\rotatebox[origin=c]{90}{1hop-2i}}} &  \href{https://www.wikidata.org/wiki/Property:P2241}{P2241} &   ${\color{red}-\phantom{0}3.56} \pm \phantom{0}8.66$ &    \href{https://www.wikidata.org/wiki/Property:P459}{P459} &             ${\color{red}-\phantom{0}6.63} \pm 14.51$ &  \href{https://www.wikidata.org/wiki/Property:P2241}{P2241} &   ${\color{red}-\phantom{0}8.57} \pm \phantom{0}7.45$ \\

&      \href{https://www.wikidata.org/wiki/Property:P17}{P17} &   ${\color{red}-\phantom{0}3.30} \pm \phantom{0}4.91$ &    \href{https://www.wikidata.org/wiki/Property:P407}{P407} &             ${\color{red}-\phantom{0}6.34} \pm 14.91$ &  \href{https://www.wikidata.org/wiki/Property:P1039}{P1039} &   ${\color{red}-\phantom{0}3.33} \pm \phantom{0}6.94$ \\

&    \href{https://www.wikidata.org/wiki/Property:P453}{P453} &   ${\color{red}-\phantom{0}2.66} \pm \phantom{0}5.26$ &  \href{https://www.wikidata.org/wiki/Property:P2241}{P2241} &   ${\color{red}-\phantom{0}3.13} \pm \phantom{0}3.40$ &      \href{https://www.wikidata.org/wiki/Property:P92}{P92} &   ${\color{red}-\phantom{0}0.70} \pm \phantom{0}2.65$ \\

&    \href{https://www.wikidata.org/wiki/Property:P518}{P518} &   ${\color{red}-\phantom{0}2.26} \pm \phantom{0}3.89$ &  \href{https://www.wikidata.org/wiki/Property:P1039}{P1039} &   ${\color{red}-\phantom{0}1.71} \pm \phantom{0}3.81$ &    \href{https://www.wikidata.org/wiki/Property:P459}{P459} &   ${\color{red}-\phantom{0}0.63} \pm \phantom{0}0.94$ \\

&  \href{https://www.wikidata.org/wiki/Property:P2715}{P2715} &   ${\color{red}-\phantom{0}0.58} \pm \phantom{0}1.49$ &      \href{https://www.wikidata.org/wiki/Property:P17}{P17} &   ${\color{red}-\phantom{0}1.17} \pm \phantom{0}2.39$ &  \href{https://www.wikidata.org/wiki/Property:P3680}{P3680} &   ${\color{red}-\phantom{0}0.40} \pm \phantom{0}1.64$ \\

&  \href{https://www.wikidata.org/wiki/Property:P1686}{P1686} &            ${\color{blue}+19.60} \pm \phantom{0}4.68$ &    \href{https://www.wikidata.org/wiki/Property:P654}{P654} &            ${\color{blue}+39.14} \pm \phantom{0}8.05$ &    \href{https://www.wikidata.org/wiki/Property:P654}{P654} &                      ${\color{blue}+32.24} \pm 13.37$ \\

&    \href{https://www.wikidata.org/wiki/Property:P531}{P531} &            ${\color{blue}+22.39} \pm \phantom{0}5.15$ &    \href{https://www.wikidata.org/wiki/Property:P837}{P837} &                      ${\color{blue}+45.34} \pm 14.07$ &    \href{https://www.wikidata.org/wiki/Property:P102}{P102} &            ${\color{blue}+39.55} \pm \phantom{0}8.56$ \\

&  \href{https://www.wikidata.org/wiki/Property:P1013}{P1013} &                      ${\color{blue}+24.53} \pm 21.48$ &    \href{https://www.wikidata.org/wiki/Property:P102}{P102} &                      ${\color{blue}+49.04} \pm 12.18$ &  \href{https://www.wikidata.org/wiki/Property:P1686}{P1686} &            ${\color{blue}+57.30} \pm \phantom{0}1.64$ \\

&    \href{https://www.wikidata.org/wiki/Property:P654}{P654} &                      ${\color{blue}+31.24} \pm 46.20$ &  \href{https://www.wikidata.org/wiki/Property:P1686}{P1686} &            ${\color{blue}+61.66} \pm \phantom{0}2.20$ &    \href{https://www.wikidata.org/wiki/Property:P805}{P805} &            ${\color{blue}+57.36} \pm \phantom{0}0.98$ \\

&    \href{https://www.wikidata.org/wiki/Property:P805}{P805} &                      ${\color{blue}+77.99} \pm 10.23$ &    \href{https://www.wikidata.org/wiki/Property:P805}{P805} &            ${\color{blue}+63.10} \pm \phantom{0}0.38$ &    \href{https://www.wikidata.org/wiki/Property:P837}{P837} &            ${\color{blue}+75.11} \pm \phantom{0}3.91$ \\

\midrule
\parbox[t]{2mm}{\multirow{10}{*}{\rotatebox[origin=c]{90}{2hop}}} &    \href{https://www.wikidata.org/wiki/Property:P453}{P453} &                       ${\color{red}-64.91} \pm 40.79$ &    \href{https://www.wikidata.org/wiki/Property:P459}{P459} &   ${\color{red}-\phantom{0}5.74} \pm \phantom{0}2.76$ &    \href{https://www.wikidata.org/wiki/Property:P453}{P453} &   ${\color{red}-\phantom{0}2.05} \pm \phantom{0}5.57$ \\

&  \href{https://www.wikidata.org/wiki/Property:P2241}{P2241} &                       ${\color{red}-10.62} \pm 50.67$ &    \href{https://www.wikidata.org/wiki/Property:P453}{P453} &             ${\color{red}-\phantom{0}5.15} \pm 12.26$ &  \href{https://www.wikidata.org/wiki/Property:P3680}{P3680} &   ${\color{red}-\phantom{0}0.33} \pm \phantom{0}0.55$ \\

&    \href{https://www.wikidata.org/wiki/Property:P102}{P102} &             ${\color{red}-\phantom{0}7.14} \pm 23.57$ &  \href{https://www.wikidata.org/wiki/Property:P1011}{P1011} &             ${\color{red}-\phantom{0}4.55} \pm 24.48$ &  \href{https://www.wikidata.org/wiki/Property:P1552}{P1552} &   ${\color{red}-\phantom{0}0.01} \pm \phantom{0}0.59$ \\

&    \href{https://www.wikidata.org/wiki/Property:P837}{P837} &   ${\color{red}-\phantom{0}1.78} \pm \phantom{0}3.14$ &  \href{https://www.wikidata.org/wiki/Property:P1706}{P1706} &   ${\color{red}-\phantom{0}0.07} \pm \phantom{0}0.89$ &  \href{https://www.wikidata.org/wiki/Property:P1012}{P1012} &  ${\color{blue}+\phantom{0}0.00} \pm \phantom{0}0.00$ \\

&    \href{https://www.wikidata.org/wiki/Property:P407}{P407} &   ${\color{red}-\phantom{0}0.91} \pm \phantom{0}4.72$ &  \href{https://www.wikidata.org/wiki/Property:P1552}{P1552} &   ${\color{red}-\phantom{0}0.05} \pm \phantom{0}0.06$ &  \href{https://www.wikidata.org/wiki/Property:P1478}{P1478} &  ${\color{blue}+\phantom{0}0.10} \pm \phantom{0}0.16$ \\

&  \href{https://www.wikidata.org/wiki/Property:P1365}{P1365} &  ${\color{blue}+\phantom{0}9.90} \pm \phantom{0}7.63$ &  \href{https://www.wikidata.org/wiki/Property:P1365}{P1365} &            ${\color{blue}+26.54} \pm \phantom{0}3.37$ &  \href{https://www.wikidata.org/wiki/Property:P2868}{P2868} &            ${\color{blue}+43.84} \pm \phantom{0}4.18$ \\

&      \href{https://www.wikidata.org/wiki/Property:P39}{P39} &                      ${\color{blue}+11.36} \pm 16.67$ &  \href{https://www.wikidata.org/wiki/Property:P1366}{P1366} &            ${\color{blue}+30.02} \pm \phantom{0}2.31$ &    \href{https://www.wikidata.org/wiki/Property:P122}{P122} &            ${\color{blue}+44.17} \pm \phantom{0}0.72$ \\

&    \href{https://www.wikidata.org/wiki/Property:P805}{P805} &            ${\color{blue}+11.56} \pm \phantom{0}2.26$ &    \href{https://www.wikidata.org/wiki/Property:P122}{P122} &            ${\color{blue}+45.00} \pm \phantom{0}0.00$ &    \href{https://www.wikidata.org/wiki/Property:P407}{P407} &            ${\color{blue}+58.38} \pm \phantom{0}7.57$ \\

&    \href{https://www.wikidata.org/wiki/Property:P531}{P531} &                      ${\color{blue}+13.35} \pm 32.37$ &  \href{https://www.wikidata.org/wiki/Property:P1686}{P1686} &            ${\color{blue}+47.00} \pm \phantom{0}0.38$ &  \href{https://www.wikidata.org/wiki/Property:P1310}{P1310} &            ${\color{blue}+64.49} \pm \phantom{0}7.77$ \\

&  \href{https://www.wikidata.org/wiki/Property:P1686}{P1686} &            ${\color{blue}+24.04} \pm \phantom{0}6.48$ &    \href{https://www.wikidata.org/wiki/Property:P837}{P837} &            ${\color{blue}+47.49} \pm \phantom{0}5.83$ &    \href{https://www.wikidata.org/wiki/Property:P837}{P837} &            ${\color{blue}+78.12} \pm \phantom{0}1.50$ \\

\midrule
\parbox[t]{2mm}{\multirow{10}{*}{\rotatebox[origin=c]{90}{2i}}} &  \href{https://www.wikidata.org/wiki/Property:P2715}{P2715} &   ${\color{red}-\phantom{0}1.93} \pm \phantom{0}5.53$ &    \href{https://www.wikidata.org/wiki/Property:P291}{P291} &   ${\color{red}-\phantom{0}0.08} \pm \phantom{0}0.18$ &  \href{https://www.wikidata.org/wiki/Property:P3680}{P3680} &   ${\color{red}-\phantom{0}0.07} \pm \phantom{0}1.16$ \\

&    \href{https://www.wikidata.org/wiki/Property:P453}{P453} &   ${\color{red}-\phantom{0}0.85} \pm \phantom{0}3.90$ &  \href{https://www.wikidata.org/wiki/Property:P3680}{P3680} &  ${\color{blue}+\phantom{0}0.00} \pm \phantom{0}0.00$ &    \href{https://www.wikidata.org/wiki/Property:P291}{P291} &   ${\color{red}-\phantom{0}0.06} \pm \phantom{0}0.09$ \\

&  \href{https://www.wikidata.org/wiki/Property:P4100}{P4100} &   ${\color{red}-\phantom{0}0.67} \pm \phantom{0}2.06$ &  \href{https://www.wikidata.org/wiki/Property:P2614}{P2614} &  ${\color{blue}+\phantom{0}0.00} \pm \phantom{0}0.00$ &    \href{https://www.wikidata.org/wiki/Property:P459}{P459} &  ${\color{blue}+\phantom{0}0.09} \pm \phantom{0}1.11$ \\

&    \href{https://www.wikidata.org/wiki/Property:P518}{P518} &   ${\color{red}-\phantom{0}0.38} \pm \phantom{0}0.56$ &    \href{https://www.wikidata.org/wiki/Property:P459}{P459} &  ${\color{blue}+\phantom{0}0.80} \pm \phantom{0}1.73$ &  \href{https://www.wikidata.org/wiki/Property:P4100}{P4100} &  ${\color{blue}+\phantom{0}1.94} \pm \phantom{0}1.30$ \\

&  \href{https://www.wikidata.org/wiki/Property:P2937}{P2937} &   ${\color{red}-\phantom{0}0.27} \pm \phantom{0}2.53$ &  \href{https://www.wikidata.org/wiki/Property:P4100}{P4100} &  ${\color{blue}+\phantom{0}1.40} \pm \phantom{0}2.41$ &      \href{https://www.wikidata.org/wiki/Property:P17}{P17} &  ${\color{blue}+\phantom{0}2.81} \pm \phantom{0}2.97$ \\

&  \href{https://www.wikidata.org/wiki/Property:P1346}{P1346} &  ${\color{blue}+\phantom{0}3.34} \pm \phantom{0}1.25$ &  \href{https://www.wikidata.org/wiki/Property:P3831}{P3831} &            ${\color{blue}+18.80} \pm \phantom{0}2.36$ &  \href{https://www.wikidata.org/wiki/Property:P2453}{P2453} &            ${\color{blue}+24.20} \pm \phantom{0}3.52$ \\

&  \href{https://www.wikidata.org/wiki/Property:P1686}{P1686} &  ${\color{blue}+\phantom{0}3.35} \pm \phantom{0}1.14$ &  \href{https://www.wikidata.org/wiki/Property:P1346}{P1346} &            ${\color{blue}+19.61} \pm \phantom{0}3.90$ &    \href{https://www.wikidata.org/wiki/Property:P642}{P642} &                      ${\color{blue}+24.98} \pm 11.04$ \\

&    \href{https://www.wikidata.org/wiki/Property:P156}{P156} &  ${\color{blue}+\phantom{0}3.42} \pm \phantom{0}2.93$ &    \href{https://www.wikidata.org/wiki/Property:P518}{P518} &            ${\color{blue}+23.39} \pm \phantom{0}4.00$ &  \href{https://www.wikidata.org/wiki/Property:P1686}{P1686} &            ${\color{blue}+29.23} \pm \phantom{0}1.98$ \\

&      \href{https://www.wikidata.org/wiki/Property:P17}{P17} &  ${\color{blue}+\phantom{0}4.08} \pm \phantom{0}5.46$ &  \href{https://www.wikidata.org/wiki/Property:P1686}{P1686} &            ${\color{blue}+29.49} \pm \phantom{0}2.32$ &  \href{https://www.wikidata.org/wiki/Property:P1264}{P1264} &                      ${\color{blue}+34.53} \pm 16.62$ \\

&    \href{https://www.wikidata.org/wiki/Property:P805}{P805} &            ${\color{blue}+34.56} \pm \phantom{0}5.43$ &    \href{https://www.wikidata.org/wiki/Property:P805}{P805} &            ${\color{blue}+34.64} \pm \phantom{0}2.82$ &    \href{https://www.wikidata.org/wiki/Property:P805}{P805} &            ${\color{blue}+35.19} \pm \phantom{0}1.50$ \\

\midrule
\parbox[t]{2mm}{\multirow{10}{*}{\rotatebox[origin=c]{90}{2i-1hop}}} &  \href{https://www.wikidata.org/wiki/Property:P2241}{P2241} &   ${\color{red}-\phantom{0}5.29} \pm \phantom{0}4.07$ &  \href{https://www.wikidata.org/wiki/Property:P1346}{P1346} &   ${\color{red}-\phantom{0}0.53} \pm \phantom{0}0.11$ &  \href{https://www.wikidata.org/wiki/Property:P3680}{P3680} &   ${\color{red}-\phantom{0}0.32} \pm \phantom{0}0.31$ \\

&    \href{https://www.wikidata.org/wiki/Property:P459}{P459} &   ${\color{red}-\phantom{0}1.81} \pm \phantom{0}7.30$ &  \href{https://www.wikidata.org/wiki/Property:P2453}{P2453} &   ${\color{red}-\phantom{0}0.05} \pm \phantom{0}0.11$ &  \href{https://www.wikidata.org/wiki/Property:P2453}{P2453} &  ${\color{blue}+\phantom{0}0.03} \pm \phantom{0}0.43$ \\

&    \href{https://www.wikidata.org/wiki/Property:P366}{P366} &   ${\color{red}-\phantom{0}0.01} \pm \phantom{0}0.02$ &  \href{https://www.wikidata.org/wiki/Property:P3680}{P3680} &  ${\color{blue}+\phantom{0}0.00} \pm \phantom{0}0.00$ &  \href{https://www.wikidata.org/wiki/Property:P1441}{P1441} &  ${\color{blue}+\phantom{0}0.40} \pm \phantom{0}1.20$ \\

&  \href{https://www.wikidata.org/wiki/Property:P3680}{P3680} &   ${\color{red}-\phantom{0}0.00} \pm \phantom{0}0.00$ &  \href{https://www.wikidata.org/wiki/Property:P1365}{P1365} &  ${\color{blue}+\phantom{0}0.00} \pm \phantom{0}0.00$ &  \href{https://www.wikidata.org/wiki/Property:P1346}{P1346} &  ${\color{blue}+\phantom{0}0.49} \pm \phantom{0}0.20$ \\

&  \href{https://www.wikidata.org/wiki/Property:P1552}{P1552} &  ${\color{blue}+\phantom{0}0.00} \pm \phantom{0}0.00$ &  \href{https://www.wikidata.org/wiki/Property:P1366}{P1366} &  ${\color{blue}+\phantom{0}0.00} \pm \phantom{0}0.00$ &  \href{https://www.wikidata.org/wiki/Property:P1552}{P1552} &  ${\color{blue}+\phantom{0}0.53} \pm \phantom{0}0.32$ \\

&  \href{https://www.wikidata.org/wiki/Property:P2868}{P2868} &  ${\color{blue}+\phantom{0}3.08} \pm \phantom{0}7.63$ &    \href{https://www.wikidata.org/wiki/Property:P805}{P805} &            ${\color{blue}+29.01} \pm \phantom{0}2.24$ &    \href{https://www.wikidata.org/wiki/Property:P131}{P131} &                      ${\color{blue}+38.66} \pm 11.83$ \\

&    \href{https://www.wikidata.org/wiki/Property:P531}{P531} &  ${\color{blue}+\phantom{0}3.60} \pm \phantom{0}2.14$ &    \href{https://www.wikidata.org/wiki/Property:P812}{P812} &            ${\color{blue}+45.54} \pm \phantom{0}6.97$ &    \href{https://www.wikidata.org/wiki/Property:P812}{P812} &            ${\color{blue}+49.94} \pm \phantom{0}5.33$ \\

&    \href{https://www.wikidata.org/wiki/Property:P131}{P131} &  ${\color{blue}+\phantom{0}3.89} \pm \phantom{0}4.81$ &      \href{https://www.wikidata.org/wiki/Property:P39}{P39} &                      ${\color{blue}+51.71} \pm 36.91$ &  \href{https://www.wikidata.org/wiki/Property:P1686}{P1686} &            ${\color{blue}+53.11} \pm \phantom{0}0.58$ \\

&    \href{https://www.wikidata.org/wiki/Property:P805}{P805} &            ${\color{blue}+10.37} \pm \phantom{0}5.57$ &  \href{https://www.wikidata.org/wiki/Property:P1686}{P1686} &            ${\color{blue}+56.63} \pm \phantom{0}0.73$ &      \href{https://www.wikidata.org/wiki/Property:P39}{P39} &                      ${\color{blue}+55.05} \pm 23.43$ \\

&  \href{https://www.wikidata.org/wiki/Property:P1686}{P1686} &            ${\color{blue}+24.58} \pm \phantom{0}6.44$ &    \href{https://www.wikidata.org/wiki/Property:P837}{P837} &                      ${\color{blue}+62.98} \pm 27.55$ &    \href{https://www.wikidata.org/wiki/Property:P837}{P837} &            ${\color{blue}+82.67} \pm \phantom{0}2.60$ \\

\midrule
\parbox[t]{2mm}{\multirow{10}{*}{\rotatebox[origin=c]{90}{3hop}}} &    \href{https://www.wikidata.org/wiki/Property:P102}{P102} &             ${\color{red}-\phantom{0}4.53} \pm 15.78$ &    \href{https://www.wikidata.org/wiki/Property:P155}{P155} &   ${\color{red}-\phantom{0}0.44} \pm \phantom{0}0.99$ &  \href{https://www.wikidata.org/wiki/Property:P3680}{P3680} &   ${\color{red}-\phantom{0}0.36} \pm \phantom{0}0.57$ \\

&    \href{https://www.wikidata.org/wiki/Property:P453}{P453} &   ${\color{red}-\phantom{0}4.23} \pm \phantom{0}2.75$ &  \href{https://www.wikidata.org/wiki/Property:P1552}{P1552} &   ${\color{red}-\phantom{0}0.16} \pm \phantom{0}0.32$ &    \href{https://www.wikidata.org/wiki/Property:P175}{P175} &   ${\color{red}-\phantom{0}0.30} \pm \phantom{0}0.46$ \\

&  \href{https://www.wikidata.org/wiki/Property:P2241}{P2241} &             ${\color{red}-\phantom{0}2.65} \pm 12.77$ &    \href{https://www.wikidata.org/wiki/Property:P937}{P937} &  ${\color{blue}+\phantom{0}0.00} \pm \phantom{0}0.00$ &  \href{https://www.wikidata.org/wiki/Property:P1441}{P1441} &   ${\color{red}-\phantom{0}0.02} \pm \phantom{0}0.04$ \\

&      \href{https://www.wikidata.org/wiki/Property:P17}{P17} &             ${\color{red}-\phantom{0}2.46} \pm 11.87$ &    \href{https://www.wikidata.org/wiki/Property:P159}{P159} &  ${\color{blue}+\phantom{0}0.00} \pm \phantom{0}0.00$ &    \href{https://www.wikidata.org/wiki/Property:P937}{P937} &  ${\color{blue}+\phantom{0}0.00} \pm \phantom{0}0.00$ \\

&    \href{https://www.wikidata.org/wiki/Property:P837}{P837} &   ${\color{red}-\phantom{0}2.14} \pm \phantom{0}3.90$ &    \href{https://www.wikidata.org/wiki/Property:P263}{P263} &  ${\color{blue}+\phantom{0}0.00} \pm \phantom{0}0.00$ &  \href{https://www.wikidata.org/wiki/Property:P1012}{P1012} &  ${\color{blue}+\phantom{0}0.00} \pm \phantom{0}0.00$ \\

&    \href{https://www.wikidata.org/wiki/Property:P531}{P531} &                      ${\color{blue}+11.21} \pm 12.84$ &  \href{https://www.wikidata.org/wiki/Property:P1366}{P1366} &            ${\color{blue}+37.92} \pm \phantom{0}2.62$ &    \href{https://www.wikidata.org/wiki/Property:P122}{P122} &            ${\color{blue}+61.14} \pm \phantom{0}0.97$ \\

&    \href{https://www.wikidata.org/wiki/Property:P768}{P768} &                      ${\color{blue}+12.08} \pm 19.51$ &    \href{https://www.wikidata.org/wiki/Property:P837}{P837} &                      ${\color{blue}+48.05} \pm 11.54$ &    \href{https://www.wikidata.org/wiki/Property:P407}{P407} &            ${\color{blue}+61.33} \pm \phantom{0}8.53$ \\

&  \href{https://www.wikidata.org/wiki/Property:P2937}{P2937} &                      ${\color{blue}+14.16} \pm 21.84$ &    \href{https://www.wikidata.org/wiki/Property:P812}{P812} &                      ${\color{blue}+50.64} \pm 11.27$ &  \href{https://www.wikidata.org/wiki/Property:P1310}{P1310} &            ${\color{blue}+65.54} \pm \phantom{0}7.14$ \\

&      \href{https://www.wikidata.org/wiki/Property:P92}{P92} &                      ${\color{blue}+16.77} \pm 14.57$ &    \href{https://www.wikidata.org/wiki/Property:P122}{P122} &            ${\color{blue}+62.28} \pm \phantom{0}0.00$ &  \href{https://www.wikidata.org/wiki/Property:P3823}{P3823} &                      ${\color{blue}+76.07} \pm 10.71$ \\

&    \href{https://www.wikidata.org/wiki/Property:P805}{P805} &            ${\color{blue}+17.95} \pm \phantom{0}2.53$ &  \href{https://www.wikidata.org/wiki/Property:P3823}{P3823} &                      ${\color{blue}+72.85} \pm 42.07$ &    \href{https://www.wikidata.org/wiki/Property:P837}{P837} &            ${\color{blue}+76.71} \pm \phantom{0}1.65$ \\

\midrule
\parbox[t]{2mm}{\multirow{10}{*}{\rotatebox[origin=c]{90}{3i}}} &    \href{https://www.wikidata.org/wiki/Property:P453}{P453} &   ${\color{red}-\phantom{0}2.18} \pm \phantom{0}4.01$ &  \href{https://www.wikidata.org/wiki/Property:P2241}{P2241} &   ${\color{red}-\phantom{0}3.44} \pm \phantom{0}4.47$ &  \href{https://www.wikidata.org/wiki/Property:P2241}{P2241} &   ${\color{red}-\phantom{0}8.03} \pm \phantom{0}5.50$ \\

&  \href{https://www.wikidata.org/wiki/Property:P2241}{P2241} &   ${\color{red}-\phantom{0}1.37} \pm \phantom{0}5.09$ &  \href{https://www.wikidata.org/wiki/Property:P4100}{P4100} &   ${\color{red}-\phantom{0}0.33} \pm \phantom{0}1.73$ &  \href{https://www.wikidata.org/wiki/Property:P3680}{P3680} &   ${\color{red}-\phantom{0}0.01} \pm \phantom{0}0.27$ \\

&  \href{https://www.wikidata.org/wiki/Property:P4100}{P4100} &   ${\color{red}-\phantom{0}0.77} \pm \phantom{0}1.09$ &  \href{https://www.wikidata.org/wiki/Property:P1534}{P1534} &   ${\color{red}-\phantom{0}0.33} \pm \phantom{0}1.13$ &    \href{https://www.wikidata.org/wiki/Property:P291}{P291} &   ${\color{red}-\phantom{0}0.00} \pm \phantom{0}0.00$ \\

&  \href{https://www.wikidata.org/wiki/Property:P2715}{P2715} &   ${\color{red}-\phantom{0}0.72} \pm \phantom{0}1.56$ &    \href{https://www.wikidata.org/wiki/Property:P291}{P291} &   ${\color{red}-\phantom{0}0.01} \pm \phantom{0}0.01$ &  \href{https://www.wikidata.org/wiki/Property:P1542}{P1542} &  ${\color{blue}+\phantom{0}0.00} \pm \phantom{0}0.00$ \\

&    \href{https://www.wikidata.org/wiki/Property:P768}{P768} &   ${\color{red}-\phantom{0}0.44} \pm \phantom{0}0.85$ &  \href{https://www.wikidata.org/wiki/Property:P3680}{P3680} &  ${\color{blue}+\phantom{0}0.00} \pm \phantom{0}0.00$ &      \href{https://www.wikidata.org/wiki/Property:P17}{P17} &  ${\color{blue}+\phantom{0}0.19} \pm \phantom{0}4.25$ \\

&    \href{https://www.wikidata.org/wiki/Property:P155}{P155} &  ${\color{blue}+\phantom{0}1.54} \pm \phantom{0}0.78$ &  \href{https://www.wikidata.org/wiki/Property:P1346}{P1346} &            ${\color{blue}+10.34} \pm \phantom{0}2.94$ &    \href{https://www.wikidata.org/wiki/Property:P805}{P805} &            ${\color{blue}+19.68} \pm \phantom{0}2.23$ \\

&    \href{https://www.wikidata.org/wiki/Property:P531}{P531} &  ${\color{blue}+\phantom{0}4.58} \pm \phantom{0}1.80$ &  \href{https://www.wikidata.org/wiki/Property:P1686}{P1686} &            ${\color{blue}+15.86} \pm \phantom{0}2.80$ &  \href{https://www.wikidata.org/wiki/Property:P1686}{P1686} &            ${\color{blue}+20.98} \pm \phantom{0}3.26$ \\

&  \href{https://www.wikidata.org/wiki/Property:P1013}{P1013} &  ${\color{blue}+\phantom{0}6.28} \pm \phantom{0}4.06$ &    \href{https://www.wikidata.org/wiki/Property:P805}{P805} &            ${\color{blue}+16.72} \pm \phantom{0}2.81$ &    \href{https://www.wikidata.org/wiki/Property:P642}{P642} &                      ${\color{blue}+22.43} \pm 15.70$ \\

&    \href{https://www.wikidata.org/wiki/Property:P805}{P805} &            ${\color{blue}+14.13} \pm \phantom{0}2.31$ &  \href{https://www.wikidata.org/wiki/Property:P3831}{P3831} &            ${\color{blue}+17.49} \pm \phantom{0}2.35$ &    \href{https://www.wikidata.org/wiki/Property:P518}{P518} &            ${\color{blue}+28.26} \pm \phantom{0}2.68$ \\

&  \href{https://www.wikidata.org/wiki/Property:P2842}{P2842} &                      ${\color{blue}+42.44} \pm 36.23$ &    \href{https://www.wikidata.org/wiki/Property:P518}{P518} &            ${\color{blue}+21.94} \pm \phantom{0}1.42$ &  \href{https://www.wikidata.org/wiki/Property:P1264}{P1264} &                      ${\color{blue}+32.88} \pm 25.04$ \\

\bottomrule

\end{tabular*}
